Understanding Generalizability of Diffusion Models Requires Rethinking the Hidden Gaussian Structure

In this work, we study the generalizability of diffusion models by looking into the hidden properties of the learned score functions, which are essentially a series of deep denoisers trained on various noise levels. We observe that as diffusion models transition from memorization to generalization, their corresponding nonlinear diffusion denoisers exhibit increasing linearity. This discovery leads us to investigate the linear counterparts of the nonlinear diffusion models, which are a series of linear models trained to match the function mappings of the nonlinear diffusion denoisers. Surprisingly, these linear denoisers are approximately the optimal denoisers for a multivariate Gaussian distribution characterized by the empirical mean and covariance of the training dataset. This finding implies that diffusion models have the inductive bias towards capturing and utilizing the Gaussian structure (covariance information) of the training dataset for data generation. We empirically demonstrate that this inductive bias is a unique property of diffusion models in the generalization regime, which becomes increasingly evident when the model's capacity is relatively small compared to the training dataset size. In the case that the model is highly overparameterized, this inductive bias emerges during the initial training phases before the model fully memorizes its training data. Our study provides crucial insights into understanding the notable strong generalization phenomenon recently observed in real-world diffusion models.

==> section3.tex <==
\section{Theoretical Analysis (Why do Diffusion Models Learn the Gaussian Structure?):}
In previous sections we've empirically showed that the diffusion models have the inductive bias towards learning the Gaussian structure of the training data. In this section, we analytically show that such structure emerges when we minimize the denoising score matching objective~\Cref{Training Denoisers} while restricting the diffusion models to be linear.

\paragraph{Setup.}
We study the problem assuming we have a finite number of training data pints $\{\mb x_1, \mb x_2,...,\mb x_N\}$, which implies that our data distribution $p_{\text{data}}(\mb x)$ is a mixture of Dirac delta distributions:
\begin{align}
    \label{eq: multi delta}
    p_{\text{data}}(\mb x)=\frac{1}{N}\sum_{i=1}^{N}\delta(\mb x-\mb x_i).
\end{align}
Suppose the denoiser $D(\mb x;\sigma)$ has \textbf{unconstrained} form, it is shown in~\cite{karras2022elucidating} that the optimal denoiser is:
\begin{align}
    D(\mb x;\sigma) = \frac{\sum_{i}\mathcal{N}(\mb x;\mb x_i,\sigma^2\mb I)\mb x_i}{\sum_{i}\mathcal{N}(\mb x;\mb x_i,\sigma^2\mb I)}.
\end{align}
However in this case since the score of the finite data points are learned perfectly, diffusion models can only generate those discrete data points, resulting in the memorization issue. On the contrary, diffusion models in practice generalize because they fail to perfectly minimize the denoising objective. To study what kind of structures can be learned in the imperfect training case, we limit the function form of the diffusion denoisers $D(\mb x;\sigma)$ as linear models (with a bias term):
\begin{align}
    D(\mb x;\sigma) = \mb W \mb x+\mb b.
\end{align}
 With this constraint, we have the following result:
\paragraph{The Optimal Linear Denoisers are Gaussian Denoisers.} Under the linear constraint, the optimal solution to~\Cref{Training Denoisers} is:
\begin{align}
    D(\mb x,\sigma)=\mb U\Tilde{\Lambda}_{\sigma}\mb U^T \mb x + (\mb I-\mb U\Tilde{\Lambda}_{\sigma}\mb U^T)\mb \mu
\end{align},
which is exactly the Gaussian denoiser. Furthermore, with a proper learning rate, this optimal solution can be achieved via gradient descent.
\paragraph{Implications:}
Our analysis implies that the diffusion models learn the Gaussian structure of the training data distribution under the linear constraint. Though in practice the diffusion models are highly nonlinear, our empirical results suggests that the diffusion models in practice have the inductive bias towards operating in such linear regime. However, we'd like to note that the images generated with the Gaussian models don’t match the perceptual quality of those generated from the diffusion models in practice which implies that nonlinearity plays an important role in image generation. We leave the investigation of nonlinearity to future work.

\begin{comment}
thereby we can simplify the training objective in~\Cref{Training Denoisers} as 
\begin{align}
    \mathcal{L}(D;\sigma) &= \mathbb{E}_{\mb x\sim p_{\text{data}}}\mathbb{E}_{\mb \epsilon\sim \mathcal{N}(\mb 0,\sigma^2\mb I)}||D(\mb x+\mb \epsilon;\sigma)-\mb x||_2^2 \\
    & =  \mathbb{E}_{\mb x\sim p_{\text{data}}}\int_{\mathbb{R}^d}\mathcal{N}(\mb \epsilon;\mb 0,\sigma^2\mb I)||D(\mb x+\mb \epsilon;\sigma)-\mb x||_2^2 d\mb \epsilon\\
    & = \frac{1}{N} \int_{\mathbb{R}^d}\sum_{i=1}^{N}\delta(\mb x-\mb x_i)\int_{\mathbb{R}^d}\mathcal{N}(\mb \epsilon;\mb 0,\sigma^2\mb I)||D(\mb x+\mb \epsilon;\sigma)-\mb x||_2^2 d\mb \epsilon d\mb x \\
    & = \frac{1}{N}\int_{\mathbb{R}^d}\mathcal{N}(\mb \epsilon;\mb 0, \sigma^2\mb I)\int_{\mathbb{R}^d}\sum_{i=1}^{N}\delta(\mb x-\mb x_i)||D(\mb x+\mb \epsilon;\sigma)-\mb x||_2^2 d\mb x d\mb \epsilon\\
    &= \frac{1}{N}\int_{\mathbb{R}^d}\mathcal{N}(\mb \epsilon;\mb 0, \sigma^2\mb I)\sum_{i=1}^{N}||D(\mb x_i+\mb \epsilon;\sigma)-\mb x_i
    ||_2^2 d\mb \epsilon \\
    \label{eq: optimizaiton problem unconstrained}
    & = \frac{1}{N}\sum_{i=1}^{N}\int_{\mathbb{R}^d}\mathcal{N}(\mb \epsilon;\mb 0, \sigma^2\mb I)||D(\mb x_i+\mb \epsilon;\sigma)-\mb x_i||_2^2\mb d\epsilon.
\end{align}
Suppose the denoiser $D(\mb x;\sigma)$ has \textbf{unconstrained} form, it is shown in~\cite{karras2022elucidating} that $\mathcal{L}(D;\sigma)$ can be minimized by minimizing $\int_{\mathbb{R}^d}\mathcal{N}(\mb \epsilon;\mb 0, \mb I)||D(\mb x_i+\mb \epsilon;\sigma)-\mb x_i||_2^2 d\mb\epsilon$ independently for each $\mb x_i$. The resulting optimal denoiser has the form:
\begin{align}
    D(\mb x;\sigma) = \frac{\sum_{i}\mathcal{N}(\mb x;\mb x_i,\sigma^2\mb I)\mb x_i}{\sum_{i}\mathcal{N}(\mb x;\mb x_i,\sigma^2\mb I)},
\end{align}
which is essentially a Softmax function over the finite data points. When $\sigma$ is small, the Softmax denosier will simply return the nearest neighbor to $\mb x$ in the training dataset, which results in the memorization phenomenon as shown in~\Cref{fig: score error and sampling trajectory} (second row in the right figure). Since the Softmax denoiser can only generate image in the training dataset, it fails to explain the generating ability of diffusion models used in practice. This is expected since in practice we only have finite number of data points. If the diffusion model learns the score of the finite data points perfectly, it can only generate those discrete data points. This issue is recently studied in the work~\cite{li2024good}, in which the authors argue that \textbf{a good score does not lead to a good generative model}. On the contrary, diffusion models generalize when they fail to perfectly minimize the denoising objective in~\Cref{Training Denoisers}. To study what kind of structures can be learned in the imperfect training case, we limit the function form of the diffusion denoisers $D(\mb x;\sigma)$ as linear models (with a bias term). 
\begin{align}
    D(\mb x;\sigma) = \mb W \mb x+\mb b.
\end{align}
In this case, we get the following optimization problem from~\Cref{eq: optimizaiton problem unconstrained}:
\begin{align}
    \label{eq: constrained optimization form}
    \mb W^\star, \mb b^\star = \argmin_{\mb W,\mb b}\mathcal{L}(\mb W,\mb b;\sigma):=\sum_{i=0}^N\int_{\mathcal{R}^d}\mathcal{N}(\mb \epsilon;\mb 0,\sigma^2\mb I)||\mb W(\mb x_i+\mb \epsilon)+\mb b-\mb x_i||_2^2 d\mb \epsilon
\end{align}

\paragraph{Result 1: The Optimal Linear Denoisers are Gaussian Denoisers.}
Notice that the optimization problem~\Cref{eq: constrained optimization form} is convex. To solve it, we first eliminate $\mb b$ by requiring the partial derivative $\nabla_{\mb b}\mathcal{L}(\mb W,\mb b;\sigma)$ to be $\mb 0$. Notice that 
\begin{align}
    \nabla_{\mb b}\mathcal{L}(\mb W,\mb b;\sigma) &= \sum_{i=1}^N\int_{\mathcal{R}^d}\mathcal{N}(\mb \epsilon;\mb 0,\sigma^2\mb I)(\mb W(\mb x_i+\mb \epsilon)+\mb b-\mb x_i) d\mb \epsilon\\
    & = \sum_{i=1}^N(\mb b+(\mb W-\mb I)\mb x_i).
\end{align}
Therefore we have
\begin{align}
    \label{eq:expression for b unconstrained}
    \mb b^\star = (\mb I-\mb W^*)\mb \mu,
\end{align}
where $\mb \mu=\frac{1}{N}\sum_{i=1}^N\mb x_i$.
Utilizing the expression for $\mb b$, we get the following equivalent form of the optimization problem~\Cref{eq: constrained optimization form}:
\begin{align}
    \mb W^\star = \argmin_{\mb W}\mathcal{L}(\mb W;\sigma):=\sum_{i=1}^N\int_{\mathcal{R}^d}\mathcal{N}(\mb \epsilon;\mb 0,\sigma^2\mb I)||\mb W(\mb x_i-\mb \mu+\mb \epsilon)-(\mb x_i-\mb \mu)||_2^2d \mb \epsilon
\end{align}
We can compute the derivative $\mathcal{L}(\mb W;\sigma)$ as:
\begin{align}
    \nabla_{\mb W}\mathcal{L}(\mb W;\sigma)&=\sum_{i=1}^{N}\int_{R^d}\mathcal{N}(\mb \epsilon;\mb 0,\mb \sigma^2\mb I)(\mb W(\mb x_i-\mb \mu)(\mb x_i-\mb \mu)^T+\mb W\mb\epsilon\mb\epsilon^T-(\mb x_i-\mb \mu)(\mb x_i-\mb \mu)^T)d\mb\epsilon\\
    &=\sum_{i=1}^{N}\mb W(\mb x_i-\mb \mu)(\mb x_i-\mb \mu)^T+N\mb W\sigma^2\mb I-\sum_{i=1}^{N}(\mb x_i-\mb \mu)(\mb x_i-\mb \mu)^T
 \end{align}.                                                                                                                                   
Furthermore, the optimal $\mb W^\star$ should satisfy $\nabla_{\mb W}\mathcal{L}(\mb W;\sigma)=\mb 0$, which leads to 
\begin{align}
    \mb W^\star(\frac{1}{N}\sum_{i=1}^{N}(\mb x_i-\mb \mu)(\mb x_i-\mb \mu)^T+\sigma^2\mb I)=\frac{1}{N}\sum_{i=0}^{N}(\mb x_i-\mb \mu)(\mb x_i-\mb\mu)^T.
\end{align}
Denote the covariance matrix of the training dataset and its singular value decomposition as:
\begin{align}
    Cov(\mb X)&=\frac{1}{N}\sum_{i=1}^N(\mb x_i-\mb \mu)(\mb x_i-\mb \mu)^T\\
    &=\mb U\mb\Lambda\mb U^T
\end{align},
 we have 
 \begin{align}
     \mb W^\star &= \mb U\mb\Lambda\mb U^T\mb U(\mb \Lambda+\sigma^2\mb I)^{-1}\mb U^T\\
     &=\mb U\Tilde{\mb\Lambda}_\sigma\mb U^T,
 \end{align}
 where $\Tilde{\mb\Lambda}_\sigma[i,i]=\frac{\lambda_i}{\lambda_i+\sigma^2}$ and $\lambda_i=\mb\Lambda[i,i]$. Substitute $\mb W^\star$ back to~\Cref{eq:expression for b unconstrained}, we have:
 \begin{align}
     \mb b^\star = (\mb I-\mb U\Tilde{\mb\Lambda}_\sigma\mb U^T)\mb \mu.
 \end{align}
 Therefore, when the diffusion denoisers are limited as linear functions, the optimal denoisers that minimize the denoising error over the empirical distribution are exactly the Gaussian denoisers. But can gradient descent recovers the optimal solution?

 \paragraph{Result 2}: Gradient Descent Recovers the Gaussian Denoisers with Proper Learning Rate.
 
 Consider minimizing the population loss in~\Cref{Training Denoisers}. Under the constraint that the denoisers are linear, we can rewrite the problem as:
 \begin{align}
 \label{eq: population risk}
     \mathcal{L}(\mb W,\mb b;\sigma):=\mathbb{E}_{\mb x\sim p_{\text{data}}}\mathbb{E}_{\mb \epsilon\sim \mathcal{N}(\mb 0,\sigma^2\mb I)}||\mb W(\mb x+\mb\epsilon)+\mb b-\mb x||_2^2.
 \end{align}
 Define $\tilde{\mathbf{W}} := \begin{bmatrix} \mathbf{W} & \mathbf{b} \end{bmatrix}$, $\tilde{\mb x}:=\begin{bmatrix} \mb x \\1\end{bmatrix}$ and $\Tilde{\mb \epsilon}=\begin{bmatrix} \mb\epsilon \\0\end{bmatrix}$, then we can rewrite~\Cref{eq: population risk} as:
 \begin{align}
 \label{eq: population risk_v2}
     \mathcal{L}(\tilde{\mb W};\sigma):=\mathbb{E}_{\mb x\sim p_{\text{data}}}\mathbb{E}_{\mb \epsilon\sim \mathcal{N}(\mb 0,\sigma^2\mb I)}||\tilde{\mb W}(\tilde{\mb x}+\Tilde{\mb\epsilon})-\mb x||_2^2.
 \end{align}
 We can compute the gradient in terms of $\tilde{\mb W}$ as:
 \begin{align}
     \nabla\mathcal{L}(\tilde{\mb W})&=2*\mathbb{E}_{\mb x, \mb \epsilon}(\Tilde{\mb W}(\Tilde{\mb x}+\Tilde{\mb \epsilon})(\Tilde{\mb x}+\Tilde{\mb \epsilon})^T-\mb x(\tilde{\mb x}+\tilde{\mb \epsilon})^T)\\
     &=2*\mathbb{E}_{\mb x, \mb \epsilon}(\tilde{\mb W}(\tilde{\mb x}\tilde{\mb x}^T+\tilde{\mb x}\tilde{\mb \epsilon}^T+\tilde{\mb \epsilon}\tilde{\mb x}^T+\tilde{\mb \epsilon}\tilde{\mb \epsilon}^T)-\mb x\tilde{\mb x}^T-\mb x\tilde{\mb \epsilon}^T).
 \end{align}
 Since $\mathbb{E}_{\mb \epsilon}(\tilde{\mb \epsilon})=\mb 0$ and $\mathbb{E}_{\mb \epsilon}(\tilde{\mb \epsilon}\tilde{\mb \epsilon}^T)=\begin{bmatrix}
     \sigma^2\mb I_{d\times d} & \mb 0_{d\times 1} \\
     \mb 0_{1\times d} & 0
 \end{bmatrix}$, we have:
 \begin{align}
     \nabla\mathcal{L}(\tilde{\mb W})&=2*\mathbb{E}_{\mb x}(\tilde{\mb W}(\tilde{\mb x}\tilde{\mb x}^T+\begin{bmatrix}
     \sigma^2\mb I_{d\times d} & \mb 0_{d\times 1} \\
     \mb 0_{1\times d} & 0
 \end{bmatrix})-\mb x\Tilde{\mb x}^T).
 \end{align}
 Since $\mathbb{E}(\tilde{\mb x}\tilde{\mb x}^T)=\begin{bmatrix}
     \mathbb{E}(\mb x \mb x^T) & \mathbb{E}(\mb x)\\
     \mathbb{E}(\mb x^T) & 1
 \end{bmatrix}$, we have:
 \begin{align}
     \nabla\mathcal{L}(\tilde{\mb W})=2\tilde{\mb W}\begin{bmatrix}
         \mathbb{E}_{\mb x}(\mb x\mb x^T)+\sigma^2\mb I &\mb u \\
         \mb u^T & 1
     \end{bmatrix}-2\begin{bmatrix}
         \mathbb{E}_{\mb x}(\mb x^T\mb x)&\mb u
     \end{bmatrix},
 \end{align}
 where $\mb \mu:=\mathbb{E}_{\mb x}(\mb x)$.
 With learning rate $\eta$, we can write the update rule as:
 \begin{align}
     \tilde{\mb W}(t+1) &=  \tilde{\mb W}(t)(1-2\eta\begin{bmatrix}
         \mathbb{E}_{\mb x}(\mb x\mb x^T)+\sigma^2\mb I &\mb u \\
         \mb u^T & 1
     \end{bmatrix})+2\eta\begin{bmatrix}
         \mathbb{E}_{\mb x}(\mb x^T\mb x)&\mb u
     \end{bmatrix}\\
     &= \tilde{\mb W}(t)(1-2\eta \mb A)+2\eta\begin{bmatrix}
         \mathbb{E}_{\mb x}(\mb x^T\mb x)&\mb u
     \end{bmatrix},
 \end{align}
 where we define $\mb A:=\mb I-2\eta\begin{bmatrix}
         \mathbb{E}_{\mb x}(\mb x\mb x^T)+\sigma^2\mb I &\mb u \\
         \mb u^T & 1
     \end{bmatrix}$
for simplicity. By recursively expanding the expression for $\tilde{\mb W}$, we have:
\begin{align}
\tilde{\mb W}(t+1)=\tilde{\mb W}(0)\mb A^{t+1}+2\eta \begin{bmatrix}
         \mathbb{E}_{\mb x}(\mb x^T\mb x)&\mb u
     \end{bmatrix}\sum_{i=0}^{t}\mb A^i.   
\end{align}
Notice that there exists a $\eta$, such that every eigen value of $\mb A$ is smaller than 1. In this case, $\mb A^{t+1}\rightarrow \mb 0$ as $t\rightarrow \infty$. Similarly, by the property of matrix geometric series, we have $\sum_{i=0}^t\mb A^i\rightarrow (\mb I-\mb A)^{-1}$. Therefore we have:
\begin{align}
    \tilde{\mb W}&\rightarrow \begin{bmatrix}
         \mathbb{E}_{\mb x}(\mb x^T\mb x)&\mb u
     \end{bmatrix} 
     \begin{bmatrix}
         \mathbb{E}_{\mb x}(\mb x\mb x^T)+\sigma^2\mb I &\mb u \\
         \mb u^T & 1
     \end{bmatrix}^{-1}\\
     &= \begin{bmatrix}
         \mathbb{E}_{\mb x}(\mb x^T\mb x)&\mb u
     \end{bmatrix} 
     \begin{bmatrix}
         \mb B &\mb u \\
         \mb u^T & 1
     \end{bmatrix}^{-1},
\end{align}
where we define $\mb B:=\mathbb{E}_{\mb x}(\mb x\mb x^T)+\sigma^2\mb I$ for simplicity. By the Sherman–Morrison–Woodbury formula, we have:
\begin{align}
    \begin{bmatrix}
         \mb B &\mb u \\
         \mb u^T & 1
     \end{bmatrix}^{-1} = \begin{bmatrix}
         (\mb B-\mb u\mb u^T)^{-1} & -(\mb B-\mb u\mb u^T)^{-1}\mb u\\
         -(1-\mb u^T\mb B^{-1}\mb u)^{-1}\mb u^T\mb B^{-1} & (1-\mb u^T\mb B^{-1}\mb u)^{-1}
     \end{bmatrix}.
\end{align}
Therefore, we have:
\begin{align}
    \tilde{\mb W}\rightarrow \begin{bmatrix}
        \mathbb{E}_{\mb x}[\mb x\mb x^T](\mb B-\mb u\mb u^T)^{-1}-\frac{\mb u\mb u^T\mb B^{-1}}{1-\mb u^T\mb B^{-1}\mb u} & -\mathbb{E}_{\mb x}[\mb x \mb x^T](\mb B-\mb u\mb u^T)^{-1}\mb u+\frac{\mb u}{1-\mb u^T\mb B^{-1}\mb u}
    \end{bmatrix},
\end{align}
from which we have 
\begin{align}
    \mb W&\rightarrow \mathbb{E}_{\mb x}[\mb x\mb x^T](\mb B-\mb u\mb u^T)^{-1}-\frac{\mb u\mb u^T\mb B^{-1}}{1-\mb u^T\mb B^{-1}\mb u}\\
        \mb b&\rightarrow-\mathbb{E}_{\mb x}[\mb x \mb x^T](\mb B-\mb u\mb u^T)^{-1}\mb u+\frac{\mb u}{1-\mb u^T\mb B^{-1}\mb u}
\end{align}
Since $\mathbb{E}_{\mb x}[\mb x\mb x^T]=\mathbb{E}_{\mb x}[(\mb x-\mb u)((\mb x-\mb u)^T]+\mb u\mb u^T$, we have:
\begin{align}
    \mb W = Cov(\mb X)(Cov(\mb X)+\sigma^2I)^{-1}+\mb u\mb u^T(\mb B-\mb u\mb u^T)^{-1}-\frac{\mb u\mb u^T\mb B^{-1}}{1-\mb u^T\mb B^{-1}\mb u}.
\end{align}
Applying Sherman-Morrison Formula, we have:
\begin{align}
    (\mb B-\mb u\mb u^T)^{-1} = \mb B^{-1}+\frac{\mb B^{-1}\mb u\mb u^T\mb B^{-1}}{1-\mb u^T\mb B^{-1}\mb u},
\end{align}
therefore
\begin{align}
    \mb u\mb u^T(\mb B-\mb u\mb u^T)^{-1}-\frac{\mb u\mb u^T\mb B^{-1}}{1-\mb u^T\mb B^{-1}\mb u} &=\frac{\mb u\mb u^T\mb B^{-1}\mb u\mb u^T\mb B^{-1}}{1-\mb u^T\mb B^{-1}\mb u}-\frac{\mb u\mb u^T\mb B^{-1}\mb u^T\mb B^{-1}\mb u}{1-\mb u^T\mb B^{-1}\mb u}\\
    &=\frac{\mb u^T\mb B^{-1}\mb u}{1-\mb u^T\mb B^{-1}\mb u}(\mb u\mb u^T\mb B^{-1}-\mb u\mb u^T\mb B^{-1})\\
    &= \mb 0
\end{align}, which implies
\begin{align}
\mb W &\rightarrow Cov(\mb X)(Cov(\mb X)+\sigma^2I)^{-1}\\
    &=\mb U\Tilde{\mb\Lambda}_\sigma\mb U^T.
\end{align}
Similarly, we have:
\begin{align}
    \mb b \rightarrow (\mb I-\mb U\Tilde{\mb\Lambda}_\sigma\mb U^T)\mb u.
\end{align}
Therefore, gradient descent with a properly chosen learning rate $\eta$ recovers the Gaussian Denoisers when time goes to infinity. Notice that this results hold for any data distribution with finite mean and covariance. 

Our analysis implies that the diffusion models learn the Gaussian structure of the training data distribution under the linear constraint. Though in practice the diffusion models are highly nonlinear, our empirical results suggests that the linear analysis still captures important characteristics of what's happening in practice, as the Gaussian model generates images that share visual similarity with those of the diffusion models in practice. However, the images generated with the Gaussian model don't match the perceptual quality of those generated from the diffusion models in practice, suggesting that nonlinearity plays an important role in image generation. We leave the investigation of nonlinearity to future work. 
\end{comment}
